Nonadaptive Learning in Robust Nonlinear Output Regulation

This paper considers robust nonadaptive regulation for general nonlinear systems in an output-feedback setting with arbitrarily high relative degree. We develop a nonadaptive design that combines an input-driven filter and a generic internal model with a recursive backstepping law, thereby recasting the regulation problem as the robust input-to-state stabilization of an augmented error system. Unlike adaptive schemes, the proposed method does not rely on linearly parameterized regressors and does not require the construction of Lyapunov functions having merely nonpositive derivatives. Under standard assumptions on the exosystem, including purely imaginary and simple eigenvalues, together with a minimum-phase input-to-state stability condition on the internal dynamics, we establish global asymptotic regulation and derive explicit, verifiable inequalities for selecting the design gains. The resulting nonadaptive framework guarantees convergence of the estimation and tracking errors even when the controlled-system dynamics are complex or only partially known. The effectiveness of the theoretical results is demonstrated using a benchmark controlled Duffing system.

==> preamble.tex <==




%\usepackage{mathbbold}
 \usepackage{amsmath}
\makeatletter
\def\underbracex#1#2{\mathop{\vtop{\m@th\ialign{##\crcr
   $\hfil\displaystyle{#2}\hfil$\crcr
   \noalign{\kern3\p@\nointerlineskip}%
   #1\crcr\noalign{\kern3\p@}}}}\limits}

\def\underbracea{\underbracex\upbracefilla}

\def\upbracefilla{$\m@th \setbox\z@\hbox{$\braceld$}%
  \bracelu\leaders\vrule \@height\ht\z@ \@depth\z@\hfill 
\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@
$}

\def\underbraceb{\underbracex\upbracefillb}

\def\upbracefillb{$\m@th \setbox\z@\hbox{$\braceld$}%
\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@
 \leaders\vrule \@height\ht\z@ \@depth\z@\hfill\bracerd
  \braceld\leaders\vrule \@height\ht\z@ \@depth\z@\hfill
\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@
$}


\def\underbracec{\underbracex\upbracefillc}

\def\upbracefillc{$\m@th \setbox\z@\hbox{$\braceld$}%
\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@
\leaders\vrule \@height\ht\z@ \@depth\z@\hfill
\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@
$}

\def\underbraced{\underbracex\upbracefilld}
\def\upbracefilld{$\m@th \setbox\z@\hbox{$\braceld$}%
\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@
 \leaders\vrule \@height\ht\z@ \@depth\z@\hfill\braceru$}

\def\underbracebd{\underbracex\upbracefillbd}
\def\upbracefillbd{$\m@th \setbox\z@\hbox{$\braceld$}%
\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@\vrule \@width\p@\kern\p@
\bracerd\braceld
 \leaders\vrule \@height\ht\z@ \@depth\z@\hfill\braceru$}


\makeatother
\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\myb}{\color{blue}}
\newcommand{\myr}{\color{red}}
%\setcitestyle{authoryear,colon}
%\usepackage[authoryear]{natbib}
%\usetikzlibrary{positioning}
%\newcounter{MYtempeqncnt}
%\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\col}{\mbox{col}}
%\renewcommand\thesection{\Roman{section}}
 
\newtheorem{Property}{Property}
\newtheorem{proposi}{Proposition}
\newtheorem{Algorithm}{Algorithm}
\newcommand{\row}{\textnormal{row}}
\definecolor{mitRed}{RGB}{117,0,20}
\definecolor{mitSilverGray}{RGB}{139,149,158}
\definecolor{mitPurple}{RGB}{153,51,255}
\definecolor{mitBlue}{RGB}{25,102,255}
\definecolor{mitGreen}{RGB}{0,173,0}
\definecolor{mitLGreen}{RGB}{170,255,51}
\definecolor{mitPink}{RGB}{255,20,240}
\definecolor{mitLightPink}{RGB}{255,179,255}
\definecolor{mitDPink}{RGB}{117,0,98}
\definecolor{mitLightBlue}{RGB}{153,235,255}
\usetikzlibrary{shapes,arrows,positioning}
%\newenvironment{Proof}{\noindent{\em Proof:\/}}{\hfill $\Box$\par}
%\newcommand{\tabref}[1]{Table~\ref{#1}}
%\captionsetup[figure]{labelfont={bf},labelformat={default},labelsep=period,name={Fig.}}
\usetikzlibrary{decorations.markings}

\tikzset{test/.style n args={3}{
    postaction={
    decorate,
    decoration={
    markings,
    mark=between positions 0 and \pgfdecoratedpathlength step 0.5pt with {
    \pgfmathsetmacro\myval{multiply(
        divide(
        \pgfkeysvalueof{/pgf/decoration/mark info/distance from start}, \pgfdecoratedpathlength
        ),
        100
    )};
    \pgfsetfillcolor{#3!\myval!#2};
    \pgfpathcircle{\pgfpointorigin}{#1};
    \pgfusepath{fill};},
  mark=at position \pgfdecoratedpathlength with {\arrow[mitDPink,line width=#1] {>}; }
}}}}
